FirmTruss Community Search in Multilayer Networks

In applications such as biological, social, and transportation networks, interactions between objects span multiple aspects. For accurately modeling such applications, multilayer networks have been proposed. Community search allows for personalized community discovery and has a wide range of applications in large real-world networks. While community search has been widely explored for single-layer graphs, the problem for multilayer graphs has just recently attracted attention. Existing community models in multilayer graphs have several limitations, including disconnectivity, free-rider effect, resolution limits, and inefficiency. To address these limitations, we study the problem of community search over large multilayer graphs. We first introduce FirmTruss, a novel dense structure in multilayer networks, which extends the notion of truss to multilayer graphs. We show that FirmTrusses possess nice structural and computational properties and bring many advantages compared to the existing models. Building on this, we present a new community model based on FirmTruss, called FTCS, and show that finding an FTCS community is NP-hard. We propose two efficient 2-approximation algorithms, and show that no polynomial-time algorithm can have a better approximation guarantee unless P = NP. We propose an index-based method to further improve the efficiency of the algorithms. We then consider attributed multilayer networks and propose a new community model based on network homophily. We show that community search in attributed multilayer graphs is NP-hard and present an effective and efficient approximation algorithm. Experimental studies on real-world graphs with ground-truth communities validate the quality of the solutions we obtain and the efficiency of the proposed algorithms.

==> Algorithm_FirmCore_G0.tex <==
\begin{algorithm}[t] 
    \small
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{An ML graph $G = (V, E, L)$, a set of query nodes $Q \subseteq V$, and integers $k$ and $\lambda$}
    \Output{A connected $(k, \lambda)$-FirmCore containing $Q$}
    $N \leftarrow \emptyset$;\\
    \ForAll{$u \in V$}{
        $I[u] \leftarrow \text{Top-$\lambda$}(\text{deg}(u))$\\
        \If{$I[u] < k$}{
            $N \leftarrow N \cup \{u\}$;
        }
    }
    \While{$N \neq \emptyset$}
    {
        Pick and remove $u$ from $N$;\\
        \ForAll{$(u, v, \ell) \in E$ and $I[v] \geq k$}{
                $\text{deg}_{\ell}(v) \leftarrow \text{deg}_{\ell}(v) - 1$;\\
                \If{$\text{deg}_{\ell}(v) = I[v] - 1$}{
                    Update $I[v]$; \\
                    \If{$I[v] < k$}{
                        $N \leftarrow N \cup \{v\}$;
                    }
                }
            }
        Remove $u$ and its incident edges from $G$;
    }
    $H \leftarrow $ The connected component of $G$ containing $Q$;\\
    \Return $H$;
    \caption{Maximal $(k, \lambda)$-FirmCore containing $Q$}
    \label{alg:FirmCore_G0}
\end{algorithm}

==> Algorithm_FirmCore_Maintenance.tex <==
\begin{algorithm}[t] 
    \small
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{An ML graph $G = (V, E, L)$, a set of nodes to be removed $V_d \subseteq V$, and integers $k$ and $\lambda$}
    \Output{A connected $(k, \lambda)$-FirmCore}
    
    \caption{FirmCore Maintenance}
    \label{alg:FirmCore_Maintenance}
\end{algorithm}

==> Algorithm_FirmTruss_Maintenance.tex <==
\begin{algorithm}[t] 
    \small
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{An ML graph $G = (V, E, L)$, a set of nodes to be removed $V_d \subseteq V$, and integers $k$ and $\lambda$}
    \Output{A connected $(k, \lambda)$-FirmTruss}
    
    \caption{FirmTruss Maintenance}
    \label{alg:FirmTruss_Maintenance}
\end{algorithm}

==> Algorithm_Maximal_FirmCore_Index.tex <==
\begin{algorithm}[t] 
    \small
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{An ML graph $G = (V, E, L)$, a set of query vertices $Q \subseteq V$, and two integers $k, \lambda$}
    \Output{A maximal connected $(k, \lambda)$-FirmCore containing $Q$}
    
    $N \leftarrow Q$;\\
    Mark all vertices of $Q$ as visited;\\
    Let $G_0$ be an empty graph;\\
    \While{$N \neq \emptyset$}{
        Pick and remove $u \in N$;\\
        \For{each unvisited node $v$ neighbours to $u$}{
            Mark $v$ as visited;\\
            \For{each skyline FirmCore index $(k_i, \lambda_i) \in \mathsf{SFC(v)}$}{
                \If{$(k, \lambda) \preceq (k_i, \lambda_i)$}{
                    add $v$ and $u$ into $G_0$;\\
                    $N \leftarrow N \cup \{ v\}$;\\
                }
            }
        }
    }
    \Return $G_0$
    \caption{Index-based Maximal FirmCore Finding}
    \label{alg:maximal_firmcore_index}
\end{algorithm}

==> Algorithm_exact_AFCCS.tex <==
\begin{algorithm}[t] 
    \small
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{An attributed ML graph $G = (V, E, L, \Psi)$, a set of query vertices $Q \subseteq V$, and two integers $k, \lambda$}
    \Output{A connected $(k, \lambda)$-FirmTruss containing $Q$ with the maximum $\Gamma_{-\infty}(.)$}
    
    $i \leftarrow 0$;\\
    $G_0 \leftarrow$ Find a maximal connected $(k, \lambda)$-FirmTruss containing $Q$; //See Algorithm~\ref{alg:maximal_firmtruss_index} \\
    Calculate $h_{V_{G_0}}(u)$ for all $u \in V_{G_0}$;\\
    
    \While{$Q \subseteq V_{G_i}$}{
        $u \leftarrow $ vertex with minimum $h_{V_{G_i}}$;\\
        $\Gamma(G_i) \leftarrow h_{V_{G_i}}(u)$;\\
        Delete vertex $u$ and its incident edges from $G_i$ in all layers;\\
        Maintain $G_i$ as $(k, \lambda)$-FirmTruss by removing vertices/edges; \\
        Let the remaining graph as $G_{i+1}$; $i \leftarrow i + 1$;
    }
    \Return $\arg \max_{H \in \{G_0, \dots, G_{i-1}\}} \Gamma_{-\infty}(H)$;
    \caption{Exact-MaxMin AFTCS}
    \label{alg:exact-AFTCS}
\end{algorithm}  

==> Algorithm_online_global_search.tex <==
\begin{algorithm}[t] 
    \small
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{An ML graph $G = (V, E, L)$, a set of query vertices $Q \subseteq V$, and two integers $k, \lambda$}
    \Output{A connected $(k, \lambda)$-FirmTruss containing $Q$ with the minimum diameter}
    
    $G_0 \leftarrow$ Find a maximal connected $(k, \lambda)$-FirmTruss containing $Q$; //See Algorithm~\ref{alg:FirmTruss_G0} \\
    $i \leftarrow 0$;\\
    
    \While{$Q \subseteq V_{G_i}$}{
        $u \leftarrow $ vertex with maximum $\text{dist}_{G_i}(u, Q)$;\\
        $\text{dist}_{G_i}(G_i, Q) \leftarrow \text{dist}_{G_i}(u, Q)$;\\
        Delete vertex $u$ and its incident edges from $G_i$ in all layers;\\
        Maintain $G_i$ as $(k, \lambda)$-FirmTruss by removing vertices/edges; \\
        Let the remaining graph as $G_{i+1}$; $i \leftarrow i + 1$;
    }
    \Return $\arg \max_{H \in \{G_0, \dots, G_{i-1}\}} \text{dist}_{H}(H, Q)$;
    \caption{FTCS Global Search}
    \label{alg:global_search}
\end{algorithm}

==> Algorithm_online_local_search.tex <==
\begin{algorithm}[t] 
    \small
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{An ML graph $G = (V, E, L)$, a set of query vertices $Q \subseteq V$, and two integers $k, \lambda$}
    \Output{A connected $(k, \lambda)$-FirmCore containing $Q$ with the minimum diameter}
    
    $G_0 \leftarrow$ Find a maximal connected $(k, \lambda)$-FirmCore containing $Q$; //See Algorithm~\ref{alg:FirmCore_G0} \\
    $i \leftarrow 1$;\\
    
    \While{$i \leq \text{dist}_{G_0}(G_0, Q)$}{
        $V' \leftarrow Q \cup \{ u \in V | \text{dist}_{G_0}(u, Q) \leq i\}$;\\
        $G' \leftarrow$ Induced subgraph of $G_0$ by vertices $V'$;\\
        Find maximal $(k, \lambda)$-FirmCore of $G'$ containing $Q$; //See Algorithm~\ref{alg:FirmCore_G0}  \\
        \While{$G' \neq \emptyset$}{
            $N \leftarrow \emptyset$;\\
            \For{$u \in V[G']$}{
                \If{$\text{dist}_{G'}(u, Q) > i$}{
                    $N \leftarrow N \cup \{ u \}$;
                }
            }
            \If{$N = \emptyset$}{
                \Return $G'$;
            }
            \Else{
                Delete~$N$~and~their~incidents~edges~in~all~layers~from~$G'$;\\
                Maintain $G'$ as $(k, \lambda)$-FirmCore;
            }
        }
        $i \leftarrow i + 1$;
    }
    \caption{FCCS Local Search}
    \label{alg:local_search}
\end{algorithm}

==> Comparision_Table.tex <==
\begin{center}
\begin{table} [tpb!]
 \caption{Comparison of CS models in multilayer networks.}
    \resizebox{0.48\textwidth}{!} {
\begin{tabular}{l | c |c |c |c }
 \toprule
  {CS Model} & {Cohesiveness} &  {Connectivity} & {Redundancy} & {Scalability}\\
 \midrule 
 \midrule
    FirmTruss                           &  $\star\star\star \:\star$  &   $\star\star\star \:\star$  &  $\star\star\star  \:\star$ & $\star\star\star$\\
    ML $\mathbf{k}$-core \cite{ml-core-journal}  &  $\star\star \star$                &  $\star$       &   $\star$ &  $\star$ \\
    ML-LCD~\cite{ML-LCD}                              &  $ \star \star$               &  $\star$  &  $\star$  & $\star\star$\\
    RWM~\cite{ML-random-walk} & $\star$ & $\star$ & $\star$ & $\star \star \star \:\star$ \\
  \toprule
\end{tabular}
}
 \label{tab:comparision_Table}
\end{table}
\end{center}
\vspace{-2ex}

==> Comparision_Table_AFCCS.tex <==
\begin{center}
\begin{table} [tpb!]
    \resizebox{0.45\textwidth}{!} {
\begin{tabular}{l | c |c |c |c | c }
 \toprule
  {CS Model} & {F1-score} &  {Density} & {Diameter} & {Size} & {Running Time (ms)}\\
 \midrule 
 \midrule
    $p = -\infty$                          & \textbf{0.64}    & \textbf{10.02}   &  \textbf{4} & 12 & \textbf{639}\\
    $p = 1$                               & \textbf{0.64}  & \textbf{10.02}   &  \textbf{4}  & 12 & 907\\
    $p = 1.5$                               & 0.619  & 8.86   &  \textbf{4}  & 13 & 990\\
    $p = 2$                               & 0.619  & 8.36   &  \textbf{4}  & 13 & 953\\
    $p = 2.5$                          & 0.59  & 8.39   &  $6$  & 20 & 876\\
    $p = 3$                           & 0.59  & 8.39   &  $6$  & 20 & 923\\
  \toprule
\end{tabular}
}
 \caption{Effect of $p$ on the quality of found community by the AFCCS method.}
 \label{tab:comparision_effectiveness_AFCCS}
\end{table}
\end{center}

==> Experiments1.tex <==
% \vspace{-2ex}
% \section{Experiments}
% \label{sec:experiments}

% In this section, we conduct experiments to evaluate our proposed model and algorithms.



% \input{Text/Data_Table}



% \vspace{-3ex}
% \head{Setup}
% All methods are implemented in Python and compiled by Cython. The experiments are performed on a Linux machine with Intel Xeon 2.6 GHz CPU and 128 GB RAM, using 4 cores in multi-core processing algorithms and using a single core otherwise. 




% \head{Baseline Methods}
%  We compare our model FCCS and FTCS with the state-of-the-art community search methods in multilayer networks. ML $\mathbf{k}$-core~\cite{ml-core-journal} uses an objective function to automatically choose a subset of layers and then find a subgraph that its minimum of minimum degrees over selected layers is maximized. ML-LCD~\cite{ML-LCD} uses a greedy strategy to find the local communities. It finds a subgraph $H$ in which the ratio of the density of links among nodes within $H$ and the density of links between nodes within $H$ and nodes outside $H$, is maximized.



% \subsection{Effectiveness Evaluation}
% In this section, we evaluate the effectiveness of proposed methods and compare them with the state-of-the-art. We use three different types of criteria to evaluate the selected methods: F1-score, diameter, and density. F1-score measures the accuracy of the detected community with regard to the ground-truth community labels. Given the discovered community $G[H]$ and the ground-truth community $G[H^*]$, F1-score is defined as:
% \begin{equation*}
%     F(H, H^*) = 2 \times \frac{prec(H, H^*) \times rec(H, H^*)}{prec(H, H^*) + rec(H, H^*)}
% \end{equation*} 
% where $prec(H, H^*) = \frac{|H\cap H^*|}{|H|}$ and $rec(H, H^*) = \frac{|H\cap H^*|}{|H^*|}$. Also, for the density, we use density measure $\rho(.)$ (Definition~\ref{dfn:density}) in multilayer networks. For each dataset, in each experiment trial, we randomly pick a set of nodes from a network as the query. To choose query nodes, we sort all vertices in descending order of their degrees in a network. A node is said to be with degree rank of $\mu\%$, if it has the top highest $\mu\%$ degree in the network. The default value is $80\%$, which means that a query node has a degree higher than the degree of $20\%$ nodes in the entire network.

% \head{Effectiveness of FCCS and FTCS}
% Table~\ref{tab:comparision_effectiveness} shows the results of the comparison of FCCS and FTCS methods with the state-of-the-art. FTCS outperforms all methods in this dataset and as is expected, FCCS is faster and outperforms others in terms of running time. The diameter of found community by ML $\mathbf{k}$-core model is disconnected and it is the reason that we have used $\infty$ in the table. Also, in comparison between our algorithms, as expected, the Hybrid algorithm is the fastest, and its quality is as good as the Local algorithm. Note that Hybrid algorithms also find each community found by Local, but because of the binary search method, the Hybrid algorithm is much faster. 

% \input{Text/Effectiveness_Table}
% \vspace{-3ex}

% Next, we test the quality of our algorithms by varying the size of the set of query nodes. Figure~\ref{fig:Quality_varying_size} shows the effect of the number of query nodes and the quality of found communities. First, increasing the size of query nodes leads to an increase in the F1 score, but after a threshold, the F1 score decreases. The reason is that by increasing the number of query nodes, they become irrelevant to each other, which may cause a decrease in the F1 score. Note that the quality of found communities by Hybrid and Local algorithms are the same.

% \input{Text/Quality_Varying_Q}

% \head{Effectiveness of AFCCS}
% In this section, we evaluate the quality of the AFCCS model. Since there are no prior algorithms for attributed community search in multilayer networks, we only compare the quality of found communities by varying $p$. As the Terrorist dataset does not have an attribute vector, we select seven layers with the minimum average degrees and embed each of them to a 10-dimensional space by node2vec~\cite{node2vec}. Then we use the average of these vectors as the attribute vector of each node. Table~\ref{tab:comparision_effectiveness_AFCCS} shows the quality of found community by AFCCS method by varying $p$. Increasing the value of $p$ increases the size of the community. Moreover, increasing the size leads to decreasing the quality. Intuitively, these results are consistant with the fact that for $p \rightarrow +\infty$, the exact solution is the maximal FirmCore, which the size is maximal and includes all free riders that may decrease the F1 score. However, note that, generally, as we discussed, the best value of $p$ is application-dependent.

% \input{Text/Comparision_Table_AFCCS}


% \vspace{-2ex}
% \subsection{Efficiency Evaluation}
% In this section, using datasets mentioned in Table~\ref{tab:datastat}, we evaluate the efficiency of our algorithms and also compare them with the state-of-the-art. 

% \head{Varying the Degree Rank of Query Nodes}
% In the first experiment, we vary the degree rank of query vertices and randomly select the query vertices from the top 20$\%$, 40$\%$, 60$\%$, 80$\%$, 100$\%$ vertices in the network. Figure~\ref{fig:varying_degree_rank} shows that all the algorithms are generally stable with respect to the varied degree of query vertices, indicating that the degree rank hardly affects the query time. 

% \input{Text/Varying_degree_rank}

% \head{Varying the Query Set Size}
% In this experiment, we vary the size of $|Q|$. Figure~\ref{fig:varying_size_Q} shows the results of this experiment. When the size of query set is increased, most of the algorithms incur a longer query time slightly. However, as expected, the index-based algorithms have consistent performance. 

% \input{Text/vary_size_Q}

% \head{Scalability}
% We evaluate the scalability of our algorithms using different versions of StackOverflow obtained by selecting a variable number of layers from 1 to 24 and also with different fractions of edges. Figure~\ref{fig:scalability} shows the results of the index construction algorithm for FirmCore and FirmTruss. As we discussed, the running time of our index-based algorithms is dominated by constructing indices. As expected, the running time scales gracefully in both directions. 

% \input{Text/Running_time_all}

% \begin{figure}[t]
%     \centering
%      \includegraphics[width=0.49\linewidth]{../Text/scalability.pdf}
%     \includegraphics[width=0.49\linewidth]{../Text/scalability2.pdf}
%     \vspace{-2ex}
%     \caption{The runtime of the FirmCore (Left) and FirmTruss (Right) index construction with varying the number of layers and the number of edges.}
%     \label{fig:scalability}
% \end{figure}



% \head{Comparative Evaluation}
% In this experiment, we compare our algorithms with the state-of-the-art in terms of the running time. The results are shown in Figure~\ref{fig:runtime_all}. FCCS algorithms outperform all other algorithms, including FirmTruss-based and state-of-the-art. As we discussed in section~\ref{sec:compare_community_models} (Table~\ref{tab:comparision_Table}), it is expected that FirmCore-based algorithms are more efficient than FirmTruss-based algorithms, while the quality of FirmTruss-based algorithms is better.   




==> FirmCommunity.tex <==
\section{Firm Community Search}
\label{sec:FirmCommunity}
In this section, we first generalize the definition of monotone and node-monotone functions to multilayer networks, and then we define the problem of \textit{FirmCommunity Search}. 


\begin{dfn}[Monotone Function]\label{dfn:Monotone-function}
Let $(V, L)$ be the tuple, representing an underlying set of nodes and a set of layers, and let $G_{(V, L)}$ be the collection of all possible ML networks defined over subsets of $V$ with set of layers $L$. Let $f: G_{(V, L)} \rightarrow \mathbb{R}$ be a function that assigns a score value to any network in $G_{(V, L)}$. We say that the function $f$ is monotone non-increasing (resp. non-decreasing) if for every graph $G \in G_{(V, L)}$ and for every induced subgraph $H$ of $G$, $f(H) \leq f(G)$ (resp. $f(H) \geq f(G)$).
\end{dfn}

\begin{dfn}[Node-monotone Function]\label{dfn:Node-Monotone-function}
Let $(V, L)$ be the tuple, representing an underlying set of nodes and a set of layers, and let $G_{(V, L)}$ be the collection of all possible ML networks defined over subsets of $V$ with set of layers $L$. Let $f: G_{(V, L)} \times V \rightarrow \mathbb{R}$ be a function that assigns a score value to any tuple in $G_{(V, L)} \times V$. The function $f$ is node-monotone non-increasing (resp. non-decreasing) if for every graph $G \in G_{(V, L)}$, for every induced subgraph $H$ of $G$, and every node $v \in H$, $f(H, v) \leq f(G, v)$ (resp. $f(H, v) \geq f(G, v)$).
\end{dfn}

Note that while $|L| = 1$, Definitions~\ref{dfn:Monotone-function}, \ref{dfn:Node-Monotone-function} are identical to the definitions of monotone and node-monotone functions in single-layer networks~\cite{k-core-community}. Following are some examples of monotone and node-monotone functions.


\begin{example}[Top-$\lambda$ Degree]
Given an integer $\lambda$, let Top$-\lambda(deg(v))$ be the $\lambda$-th largest value in the degree vector of node $v$, function Top$-\lambda(deg(.))$ is node-monotone. Also, let $f(H)$ be the minimum Top$-\lambda(deg(v))$ of any node $v \in H$, the function $f$ is monotone.
\end{example}

When a node-monotone function $f$ is boolean (its output is either 0 or 1), we refer to it as a property. We abuse the notation $f_{\ell}(H, v) = f(G_\ell[H], v)$, where $H \subseteq V$ and $v \in V$, to show the value of $f(H, v)$ in layer $\ell$.

\begin{dfn}[Node-Property Support]
Let $G = (V, E, L)$ be an ML network, $f$ be a property function, $H \subseteq V$, and $v \in H$, property support of $f(H, v)$, $PS_H(f, v)$, is the number of layers $\ell \in L$ that $f_\ell(H, v) = 1$:
\begin{equation*}
PS_H(f, v) = \sum_{\ell = 1}^{|L|} f_\ell(H, v).
\end{equation*}
\end{dfn}

\eat{Before defining the FirmCommunity Search problem, we need to define the optimum of node-monotone functions over all subgraphs of a network. Let $f: G_{(V, L)} \times V \rightarrow \mathbb{R}$ be a node-monotone function, we say $G[H] \subseteq G$ maximize (resp. minimize) the function $f$ over all subgraphs of $G$, if $\min_{v \in H} f(G[H], v) \geq \min_{v \in H'} f(G[H'], v)$ (resp. $\max_{v \in H} f(G[H], v) \leq \max_{v \in H'} f(G[H'], v)$), for all $G[H'] \subseteq~G$.
}

% \begin{tcolorbox}
\begin{problem}[FirmCommunity Search]
Given an ML network $G = (V, E, L)$, a set of query vertices $Q \subseteq V$, a monotone function $f: G_{(V, L)} \rightarrow \mathbb{R}$, a set of properties $\{p_1, p_2, \dots, p_k\}$, and a set of integers $\{\lambda_1, \dots, \lambda_k\}$, find a connected subgraph $G[H] \subseteq G$ such that:
\begin{enumerate}
    \item $Q \subseteq H$,
    \item $\forall \:\: 1 \leq i \leq k, v \in V  : PS_H(p_i, v) \geq \lambda_i$,
    \item minimize (maximize) function $f$. 
\end{enumerate}
\end{problem}
% \end{tcolorbox}


\eat{\subsection{Exact Algorithm}}


==> FirmCommunity_Undirected.tex <==
\section{FirmCommunity Variants }
\label{sec:FirmCommunity-Variants }
In this section, we discuss two variants and special cases of the FirmCommunity Search problem.  
\subsection{FirmCore-Based Community Search}
\label{sec:undirected-firmcore-based-community-search}
In this section, we develop a variant of FirmCommunity based on FirmCore structure in multilayer networks. $(k, \lambda)$-FirmCore is a maximal subgraph in which each node in at least $\lambda$ layers has a degree of at least $k$ within the subgraph. In this model, we identify a community as a group of nodes in which each node has a sufficient number of connections in a sufficient number of layers. 

\begin{dfn}[FirmCore]\label{dfn:FirmCore}
Given an undirected ML graph $G$, an integer threshold $1 \leq  \lambda \leq |L|$, and an integer $k \geq 0$, the $(k, \lambda)$-FirmCore of $G$ ($(k, \lambda)$-FC for short) is a maximal subgraph $H = G[C_{k}] = (C_{k}, E[C_{k}], L)$ such that for each node $v\in C_k$ there are at least $\lambda$ layers $\{\ell_1, ..., \ell_\lambda\} \subseteq L$ such that $\text{deg}^H_{\ell_i}(v) \geq k$, $1\leq i\leq \lambda$.
\end{dfn}


Next we formally define the problem of FirmCore Community Search. 

\begin{problem}[FirmCore Community Search] Given an ML network $G = (V, E, L)$, two integers $k, \lambda \geq 0$, and a set of query vertices $Q \subseteq V$, the FirmCore community search (FCCS) is to find a connected subgraph $G[H] \subseteq G$ satisfying:
\begin{enumerate}
    \item $Q \subseteq H$,
    \item $G[H]$ is a $(k, \lambda)$-FirmCore,
    \item diameter of $G[H]$ should be the minimum among all subgraphs satisfying conditions (1) and (2).
\end{enumerate}
\end{problem}
In the definition, condition (1) requires that the community contains the query vertex set Q, condition (2) makes sure that the community should be densely connected through a sufficient number of layers, condition (3) requires that each vertex in the community should be as close to other vertices as possible, which excludes irrelevant vertices from the answer. Together, all three conditions ensure that the returned community is a cohesive subgraph with good quality.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\linewidth]{Text/truss3.pdf}
    \caption{An example of multilayer collaboration network}
    \label{fig:CommunitySearch_example}
\end{figure}

\begin{example}
Let $k = 3$ and $\lambda = 2$, the entire graph shown in Figure~\ref{fig:CommunitySearch_example} is a $(k, \lambda)$-FirmCore. Let $v_1$ be the query node, the FCCS community removes red nodes due to their distance to $v_1$. The union of blue nodes and black node is $(3, 2)$-FirmCore as well but has smallest diameter than the entire graph.
\end{example}

\head{Hardness Analysis} Next we analyze the hardness of the FCCS problem and show that not only it is NP-hard but also is APX-hard and cannot be approximated within a factor better than $2 - \epsilon$. Thereto, we define the decision version of the FCCS, $d$-FCCS, to test whether $G$ contains a connected FirmCore community with diameter at most $d$, that contains $Q$. Following results show that not only in general FCCS problem is NP-hard but also for any arbitrary value of $\lambda$ and $|L|$ it is NP-hard.


\begin{theorem}[$d$-FCCS Hardness] \label{theorem:FCCS-hardness}
The $d$-FCCS problem is NP-hard.
\end{theorem}

\begin{proof}
We reduce the well-known NP-hard problem of Maximum Clique (decision version) to $d$-FCCS problem. Given a single-layer graph $G = (V, E)$ and integer $k$, the Maximum Clique Decision problem is to check whether $G$ contains a clique of size $k$. From this, construct an instance $G' = (V', E', L)$, where $V' = V$, $|L|$ is an arbitrary number $\geq \lambda$, $E'_\ell = E$ for each $\ell \in \hat{L} = \{\ell_1, \dots, \ell_\lambda \}$ and $E'_\ell = \emptyset$ for $\ell \in L/\hat{L}$, parameters $k$ and $d = 1$, and the empty set of query nodes $Q = \emptyset$. We show that the instance of the Maximum Clique (decision version) problem is a YES-instance iff the corresponding instance of $d$-FCCS problem is a YES-instance.

$(\Rightarrow) \: :$ A set of vertices $H \subseteq V$ that in any layer $\ell \in \hat{L}$ is a clique with at least $k$ vertices is a connected $(k-1, \lambda)$-FirmCore with diameter 1 since each node has at least $k - 1$ neighbours in $\lambda$ layers. 

$(\Leftarrow) \: :$ Given a solution $H$ for $d$-FCCS problem, so each vertex in at least $\lambda$ layers has degree at least $k - 1$, but since for $\ell \in L/\hat{L}$ the set of edges in layer $\ell$ is empty, all vertices each in layers $\ell \in \hat{L}$ has degree at least $k - 1$. Given a layer $\ell \in \hat{L}$, the distance of two arbitrary nodes $v \neq u \in V'$, in $G'_\ell[H]$ is 1 since if their shortest path contains an inter-layer edge, then its length is at least 2. Therefore, $G_\ell[H]$ contains a clique of size at least $k$.
\end{proof}

Given the NP-hardness of the FCCS problem, it is worth considering if it may be approximated. The following is an analysis of approximation and non-approximability.

\head{Hardness of Approximation} Given $\alpha \geq 1$, an algorithm achieves an $\alpha$-approximation to FCCS problem if it outputs a connected $(k, \lambda)$-FirmCore, $G[H]\subseteq G$, such that $Q \in H$ and $diam(G[H]) \leq \alpha \times diam(G[H^*])$, where $G[H^*]$ is the optimal solution to FCCS problem.

\begin{theorem} [FCCS Non-Approximability]\label{theorem:FCCS-apx}
Unless $P = NP$, for any $\epsilon > 0$, the FCCS-problem cannot be approximated in polynomial-time within a factor $(2 - \epsilon)$ of the optimal solution.
\end{theorem}

\begin{proof}
We prove it by contradiction. Assume that there exists a $(2 - \epsilon)$-approximation algorithm for the FCCS problem in polynomial-time complexity, no matter how small the $\epsilon \in (0, 1)$ is. Therefore, there is an algorithm $\mathcal{A}$ that provides a solution $H$ with an approximation factor $(2 - \epsilon)$ of the optimal solution $H^*$. Let the set of query nodes empty $Q = \emptyset$, $G = (V, E)$ be an instance of Maximum Clique Decision problem, and construct $G' = (V', E', |L|)$, where $V' = V$, $|L| = \lambda$, and for each $\ell \in L : E'_\ell = E$. We claim that $G$ contains a clique of size $k$ iff $\mathcal{A}$ outputs a solution $H$ that is $(k - 1, \lambda)$-FirmCore with diameter 1. 

$(\Rightarrow) \: :$ Clearly, if $\mathcal{A}$ outputs a solution $G'[H]$ that is $(k-1, \lambda)$-FirmCore with diameter 1, then $G_\ell[H]$ is a clique of size at least $k$ for each $\ell \in L$.

$(\Leftarrow) \: :$ Suppose $diam(G'[H]) \geq 2$, so:
\begin{equation*}
    2 diam(G[H^*]) > (2 - \epsilon) diam(G[H^*]) \geq diam(G[H]) \geq 2. 
\end{equation*}
Since diameter is an integer, we deduce that $diam(H^*) \geq 2$. In this case, $G$ cannot possibly contain a clique of size $k$, for if it did, that clique would be the optimal solution to the FCCS problem with diameter of 1. Therefore, we can distinguish between the YES and NO instances of the Maximum Clique Decision problem in polynomial-time, which is contradiction. 
\end{proof}

\head{Free-rider Effect} As discussed in Section~\ref{sec:preliminaries}, there is an undesirable phenomenon called the “free-rider effect,” which corresponds to admitting irrelevant subgraphs in the detected community. In the following, we show that FCCS-problem avoids the problem of the free-rider effect.

\begin{theorem}[FCCS Free-Rider Effect]\label{theorem:FCCS-free-rider}
For any multilayer network $G = (V, E, L)$ and query vertices $Q \subseteq V$, there is a solution $G[H]$ to the FCCS problem such that for all query-independent optimal solutions $G[H^*]$, either $H^* = H$, or $G[H \cup H^*]$ is disconnected, or $G[H \cup H^*]$ has a strictly larger diameter than $G[H]$.
\end{theorem}

\begin{proof}
Let $G[H]$ be the maximal subgraph among all optimal solutions to the FCCS problem, and $G[H^*]$ be any query-independent optimal solution. We prove this theorem by contradiction. If $G[H] \neq G[H^*]$, $G[H \cup H^*]$ is a connected $(k, \lambda)$-FirmCore containing $Q$, and $diam(G[H \cup H^*]) \leq diam(G[H])$, then $G[H \cup H^*]$ is an optimal solution to the FCCS problem while $G[H] \subseteq G[H \cup H^*]$, violating the maximality of $G[H]$.
\end{proof}





\subsection{FirmTruss-Based Community Search}
% \label{sec:undirected-firmtruss-based-community-search}



\begin{problem}[FirmTruss Community Search] Given an ML network $G = (V, E, L)$, two integers $k, \lambda \geq 0$, and a set of query vertices $Q \subseteq V$, the FirmTruss community search (FTCS) is to find a connected subgraph $G[H] \subseteq G$ satisfying:
\begin{enumerate}
    \item $Q \subseteq H$,
    \item $G[H]$ is a $(k, \lambda)$-FirmTruss,
    \item diameter of $G[H]$ should be the minimum among all subgraphs satisfying conditions (1) and (2).
\end{enumerate}
\end{problem}


\begin{example}
Let $k = 4$ and $\lambda = 1$, the union of blue and red nodes in the graph shown in Figure~\ref{fig:CommunitySearch_example} is a $(k, \lambda)$-FirmTruss. Let $v_1$ be the query node, the FTCS community removes red nodes due to their distance to $v_1$. 
\end{example}

\head{Hardness Analysis} In the following, we analyze the hardness of the FTCS problem and show that it is NP-hard and also APX-hard. Similar to the hardness analysis of FCCS problem, we define the decision version of the FTCS, $d$-FTCS, to test whether $G$ contains a connected FirmTruss community with diameter at most $d$, that contains $Q$.


\begin{theorem}[$d$-FTCS Hardness]\label{theorem:FTCS-hardness}
The $d$-FTCS problem is NP-hard.
\end{theorem}


\begin{theorem} [FTCS Non-Approximability]\label{theorem:FTCS-apx}
Unless $P = NP$, for any $\epsilon > 0$, the FTCS-problem cannot be approximated in polynomial-time within a factor $2 - \epsilon$ of the optimal solution.
\end{theorem}


\begin{theorem}[FTCS Free-Rider Effect]\label{theorem:FTCS-free-rider}
For any multilayer network $G = (V, E, L)$ and query vertices $Q \subseteq V$, there is a solution $G[H]$ to the FTCS problem such that for all query-independent optimal solutions $G[H^*]$, either $H^* = H$, or $G[H \cup H^*]$ is disconnected, or $G[H \cup H^*]$ has a strictly larger diameter than $G[H]$.
\end{theorem}


The proofs of Theorems~\ref{theorem:FTCS-hardness}, \ref{theorem:FTCS-apx}, \ref{theorem:FTCS-free-rider} are analogous to the proof of Theorems~\ref{theorem:FCCS-hardness}, \ref{theorem:FCCS-apx}, \ref{theorem:FCCS-free-rider} , respectively.









\subsection{Algorithms}\label{sec:algorithm}
Given the hardness of the FCCS and FTCS problems, in this section, we propose three efficient 2-approximation algorithms and a fast heuristic algorithm. Then we discuss an index construction method to speed up these algorithms. 


\subsubsection{Online Global Search Algorithms}
This section presents the first algorithm, called Global. We start by giving a definition of query distance in multilayer networks.

\begin{dfn}[Query Distance]
Given an multilayer network $G = (V, E, L)$, a subgraph $G[H] \subseteq G$, a set of query vertices $Q \subseteq H$, and a vertex set $S \subseteq H$, the query distance of $S$ in $G[H]$, $dist_{G[H]}(S, Q)$, is defined as the maximum length of the shortest path from $u \in S$ to a query vertex $q \in Q$, i.e., $dist_{G[H]} (S, Q) = \max_{u \in S, q \in Q} dist(u, q)$.
\end{dfn}

For simplicity, we use $dist_{G}(u, Q)$ to represent the query distance for a vertex $u \in V$. Motivated by~\cite{closest}, we develop a greedy algorithm to find a connected FirmCore (FirmTruss) with the smallest diameter. Here is an overview of the algorithm. Given integers $k$ and $\lambda$, it first finds the maximal connected $(k, \lambda)$-FirmCore (resp. $(k, \lambda)$-FirmTruss) containing $Q \subseteq V$, denoted as $G_0$. Since the diameter of $G_0$ may be large, it then iteratively removes the vertices far away to $Q$ and maintains the remaining graph as a $(k, \lambda)$-FirmCore (resp. $(k, \lambda)$-FirmTruss).

\head{FCCS Global Algorithm}
We present the details of FCCS global algorithm in Algorithm~\ref{alg:global_search}. It first finds $G_0$ that is a maximal connected $(k, \lambda)$-FirmCore containing $Q$. Then in each iteration, in line 4, for each vertex $u \in V[G_i]$, we compute the distance between $u$ and query vertex set $Q$ to obtain the query distance and delete the vertex with maximum query distance and all its incident edges in all layers. Then in the resulted graph $G_i$ we remove edges/vertices to maintain $G_i$ as a $(k, \lambda)$-FirmCore (lines 7 and 8). We maintain the $(k, \lambda)$-FirmCore by deleting the nodes whose Top-$\lambda$ degree is smaller than $k$. Finally, the algorithm terminates and returns a subgraph $G^*$, where $G^* \in \{ G_0, G_1, \dots, G_{i - 1} \}$, with the smallest query distance, $dist_{G_i}(V[G_i], Q)$.


%%%%%%%%%% Online Global Algorithm %%%%%%%%%% 
\input{Text/Algorithm_online_global_search}

The procedure of finding the maximal FirmCore containing $Q$ is elaborated in Algorithm~\ref{alg:FirmCore_G0}. Recall the definition of $(k, \lambda)$-FirmCore (Definition~\ref{dfn:FirmCore}) states that $(k, \lambda)$-FirmCore is a maximal subgraph $G[C^\lambda_k]$ in which each vertex $v \in C^\lambda_k$ has Top-$\lambda$ degree at least $k$. Thus, the algorithm first iteratively deletes all disqualified vertices and their incident edges from the original graph $G$, and then update the degree of their neighbours. To efficiently update the Top-$\lambda$ degree of their neighbours, we use the fact that if $u$ and $v$ are neighbours in layer $\ell$, removing $v$ cannot affect the top-$\lambda$ degree of $u$, unless Top-$\lambda(deg(u)) = deg_\ell(u)$. Thus, in line 11 we update the Top-$\lambda$ degree of nodes that removing $v$ may affect their Top-$\lambda$ degree. Finally, we use BFS traversal from a query node $q \in Q$ to find the connected component including query vertices. Note that the step of FirmCore maintenance in Algorithm~\ref{alg:global_search} (line 7) can use the similar operations shown in the lines 6-14 of Algorithm~\ref{alg:FirmCore_G0}. Therefore, the details of FirmCore maintenance are omitted in this paper. Next, we analyze the quality approximation and complexity of the FCCS Global algorithm.

%%%%%%%%%% FirmCore G_0 Algorithm %%%%%%%%%% 
\input{Text/Algorithm_FirmCore_G0}


\begin{theorem}[FCCS-Global Quality Approximation]\label{theorem:FCCS-Global-approx-quality}
Algorithm~\ref{alg:global_search} achieves 2-approximation to an optimal solution $G[H^*]$ of the FCCS problem, that is, the obtained $(k, \lambda)$-FirmCore, $G[H]$, has \begin{equation*}
    diam(G[H])\leq 2 \times diam(G[H^*]).
\end{equation*}
\end{theorem}

\begin{proof}
Motivate by~\cite{closest}, we first prove: 
\begin{equation*}
dist_{G[H]}(H, Q) \leq dist_{G[H^*]}(H^*, Q).
\end{equation*}
Algorithm~\ref{alg:global_search} outputs a sequence of intermediate graphs\\ $\hat{G} = \{G_0, G_1, \dots, G_{i - 1}\}$, which are $(k, \lambda)$-FirmCores containing query vertices $Q$. Therefore, we have $G_{i - 1} \subseteq \dots \subseteq G_{1} \subseteq G_0 \subseteq G$ and also since the optimal solution is also a $(k, \lambda)$-FirmCore, $G[H^*] \subseteq G_0$. We consider two cases: 

\textbf{(I)} $G[H^*] \nsubseteq G_{i - 1}$. Suppose the first deleted vertex $u^* \in H^*$ happens in graph $G_s$, this vertex must be deleted because of the distance constraint but not the FirmCore structure maintenance. Accordingly, $dist_{G_s}(G_s, Q) = dist_{G_s}(u^*, Q) = dist_{G_s}(H^*, Q)$. Since $H$ has the smallest query distance in $\hat{G}$ and $G[H^*] \subseteq G_s$, we have:
\begin{equation*}
    dist_{G[H]}(H, Q) \leq dist_{G_s}(G_s, Q) = dist_{G_s}(H^*, Q) \leq dist_{G[H^*]}(H^*, Q)
\end{equation*}

\textbf{(II)} $G[H^*] \subseteq G_{i - 1}$. We prove this case by contradiction. Assume that $dist_{G_{i - 1}}(G_{i - 1}, Q) > dist_{G_{i - 1}}(H^*, Q)$, then there exist a vertex $u^* \in G_{i - 1}\char`\\H^*$ with the largest query distance $dist_{G_{i-1}}(u^*, Q) = dist_{G_{i-1}}(G_{i-1}, Q) > dist_{G_{i - 1}}(H^*, Q)$. In the next iteration, Algorithm~\ref{alg:global_search} will delete $u^*$ from $G_{i-1}$, and maintain the FirmCore structure of $G_{i-1}$. Since $G[H^*] \subseteq G_{i - 1}$, the output of this iteration is a feasible FirmCore. This contradicts that $G_{i-1}$ is the last feasible FirmCore. Therefore, 
\begin{align*}
     & \:\: \: dist_{G[H]}(H, Q) \leq dist_{G_{i-1}}(G_{i-1}, Q)\leq dist_{G_{i-1}}(H^*, Q)\\
     & \leq dist_{G[H^*]}(H^*, Q).
\end{align*}
From above we have proved that $dist_{G[H]}(H, Q) \leq dist_{G[H^*]}(H^*, Q)$. Not that based on the triangle inequality  
\begin{equation*}
    diam(G[H]) \leq 2dist_{G[H]}(H, Q).
\end{equation*}
Thus, we can conclude that:
\begin{equation*}
    diam(G[H]) \leq 2dist_{G[H]}(H, Q) \leq 2 dist_{G[H^*]}(H^*, Q).
\end{equation*}
\end{proof}




\begin{lemma}\label{lemma:time_complexity_FirmCore}
Algorithm~\ref{alg:FirmCore_G0} takes $\mathcal{O}\left(|V|\lambda \log|L| + (|V|+ |E|)|L| \right)$ time, and $\mathcal{O}(|E| + |V||L|)$ space. 
\end{lemma}
\begin{proof}
Using a heap, we can find the $\lambda$-th largest element of degree vector in $\mathcal{O}(|L|+\lambda \log|L|)$ time so lines 2-5 take $\mathcal{O}(|V|( |L| + \lambda\log |L|))$ time. We remove each vertex at most one time from $N$, taking time $\mathcal{O}(|V|)$, and each edge is counted once, taking time $\mathcal{O}(|E|)$ (lines 8-9). Finally, to update the buckets for a given node we need $\mathcal{O}(|L|)$, so line 11 takes $\mathcal{O}(|E| |L|)$ time. Also, it needs to store Top-$\lambda$ degree of all vertices (line 3) as well as the set of edges (line 8). Thus, it needs $\mathcal{O}(|V||L| + |E|)$ space.
\end{proof}

\begin{theorem}[FCCS-Global Complexity]
Algorithm~\ref{alg:global_search} takes\\ $\mathcal{O}(t(|V_0| + |E_0|)+|V|\lambda\log|L|+(|V|+|E|)|L|)$ time, and $\mathcal{O}(|V||L| + |E|)$ space, where $t$ is the number of iterations, $V_0$ and $E_0$ are the vertex set and edge set of maximal $(k, \lambda)$-FirmCore. 
\end{theorem}

\begin{proof}
The time complexity of finding $G_0$ is $\mathcal{O}(|V|\lambda \log|L| + (|V|+ |E|)|L|)$ (Lemma~\ref{lemma:time_complexity_FirmCore}). Let $t$ be the number of iterations, and $V_0$ and $E_0$ be the vertex set and edge set of $G_0$. The computation of shortest distances by a BFS traversal starting from each query vertex $q \in Q$ takes $\mathcal{O}(t|Q||E_0|)$. The time complexity of maintenance algorithm is $\mathcal{O}(t|V_0| + |E_0|)$ in $t$ iterations, since each edge in $G_0$ is removed at most one time in all iteration and in each iteration we need to check the Top-$\lambda$ degree of each vertex. Note that, in this process we do not need to re-compute the Top-$\lambda$ degree of each node. Since in each iteration we delete at least one node and its incident edges in all layers, which is at least $(k-1)
\times \lambda$, the total number of iterations $t$ is $\mathcal{O}(\min \{|V_0| - k, \frac{|E_0|}{\lambda . k} \} )$. The space complexity of Algorithm~\ref{alg:global_search} is dominated by finding $G_0$, which takes $\mathcal{O}(|V||L| + |E|)$ space (Lemma~\ref{lemma:time_complexity_FirmCore}).
\end{proof}


\head{FTCS Global Algorithm}
The overall procedure of the FTCS-Global algorithm is exactly the same as Algorithm~\ref{alg:global_search} when in lines 1 and 7 we use FirmTruss structure instead of FirmCore. Therefore, the pseudocode of FTCS-Global Algorithm is omitted in this
paper.

The procedure of finding the maximal FirmTruss containing $Q$ is elaborated in Algorithm~\ref{alg:FirmTruss_G0}. Recall the definition of $(k, \lambda)$-FirmTruss (Definition~\ref{dfn:FirmTruss}) states that $(k, \lambda)$-FirmTruss is a maximal subgraph $G[J^\lambda_k]$ in which each edge schema $\varphi \in \mathcal{E}[J^\lambda_k]$ has Top-$\lambda$ support at least $k - 2$. The algorithm first use the following lemma.

\begin{lemma}
Given a multilayer network $G = (V, E, L)$, and two integers $k, \lambda$, the $(k, \lambda)$-FirmTruss of $G$ is a subgraph of $(k - 1,\lambda)$-FirmCore of $G$.
\end{lemma}
\begin{proof}
Given an edge schema $(v, u) \in \mathcal{E}$, where $u, v \in V$, since $(v, u)$ in at least $\lambda$ layers has at least $k - 2$ supports, $u$ and $v$ each has degree at least $k - 1$ in at least $\lambda$ layers.
\end{proof}

Thus, the algorithm first find the $(k-1, \lambda)$-FirmCore and then compute the edges' support. It then iteratively deletes all instance of disqualified edge schemas in all layers from the original graph $G$, and then update the support of their adjacent edges. To efficiently update the Top-$\lambda$ support of their adjacent edges, we use Fact~\ref{fact:FirmTruss_algorithm2}. Thus, in lines 14-17 we update the Top-$\lambda$ support of edge schemas that removing $\varphi$ may affect their Top-$\lambda$ support. Finally, we use BFS traversal from a query node $q \in Q$ to find the connected component including query vertices. Similar to maintenance of FirmCore, we omit the details of FirmTruss maintenance since it can use the similar operations shown in the lines 8-21 of Algorithm~\ref{alg:FirmTruss_G0}. Next, we analyze the quality approximation and complexity of the FTCS Global algorithm.

%%%%%%%%%% FirmTruss G_0 Algorithm %%%%%%%%%% 
\input{Text/Algorithm_FirmTruss_G0}

\begin{theorem}[FTCS-Global Quality Approximation]
Algorithm~\ref{alg:global_search} achieves 2-approximation to an optimal solution $G[H^*]$ of the FTCS problem, that is, the obtained $(k, \lambda)$-FirmTruss, $G[H]$, has \begin{equation*}
    diam(G[H])\leq 2 \times diam(G[H^*]).
\end{equation*}
\end{theorem}

\begin{proof}
The crux of the proof is similar to the Theorem~\ref{theorem:FCCS-Global-approx-quality}'s.
\end{proof}




\begin{lemma}\label{lemma:time_complexity_FirmTruss}
Algorithm~\ref{alg:FirmTruss_G0} takes $\mathcal{O}(\sum_{\ell \in L} |E_\ell|^{1.5} + |E||L| + |E|\lambda \log |L|)$ time, and $\mathcal{O}(|E||L|)$ space. 
\end{lemma}
\begin{proof}
The proof is analogous to analysis of time complexity of Algorithm~\ref{alg:FirmTruss_decomposition} in Section~\ref{sec:algorithm_FirmTruss}.
\end{proof}

\begin{theorem}[FTCS-Global Complexity]
FTCS-Global algorithm takes $\mathcal{O}(t (|Q| |E_0| + \sum_{\ell \in L} |E_\ell|^{1.5}) + |E||L| + |E|\lambda \log |L|)$ time, and $\mathcal{O}(|E||L|)$ space.
\end{theorem}

\begin{proof}
First, Algorithm 1 finds the maximal $(k, \lambda)$-FirmTruss of $G$, which takes $\mathcal{O}(\sum_{\ell \in L} |E_\ell|^{1.5} + |E||L| + |E|\lambda \log |L|)$ time as analyzed in Lemma~\ref{lemma:time_complexity_FirmTruss}. Then, it
iteratively deletes the vertex with the largest query distance starting from $G_0$ with $|E_0|$ edges. In each iteration, the algorithm needs to compute the query distance using $\mathcal{O}(|Q| |E_0|)$ time and to perform FirmTruss maintenance using $\mathcal{O}(\sum_{\ell \in L} |E_\ell|^{1.5})$. Therefore, for $t$ iterations the time cost is $\mathcal{O}(t (|Q| |E_0| + \sum_{\ell \in L} |E_\ell|^{1.5}))$. In total, FTCS-Global algorithm takes $\mathcal{O}(t (|Q| |E_0| + \sum_{\ell \in L} |E_\ell|^{1.5}) + |E||L| + |E|\lambda \log |L|)$ time. The space complexity of FTCS-Global algorithm is dominated by finding $G_0$, which takes $\mathcal{O}(|E||L|)$ space (Lemma~\ref{lemma:time_complexity_FirmTruss}).
\end{proof}


\head{FCCS Binary Search Algorithm}
We propose an optimization technique by binary search to accelerate the process of FCCS- and FTCS-Global algorithms. Algorithm~\ref{alg:global_search} as well as FTCS-Global algorithm can progressively converge to the minimum query distance. However, the algorithm reduces the query distance at most by 1 in each iteration, which is not efficient. To address this deficiency, we employ a binary search technique to speed up the process. 

%%%%%%%%%% Binary Search Online Global Algorithm %%%%%%%%%% 
\input{Text/Algorithm_binary_search_global}

Algorithm~\ref{alg:binary_search} outlines using binary search in the Global algorithm. It first finds $G_0$ that is a maximal connected $(k, \lambda)$-FirmCore containing $Q$. Then it uses the maximum query distance in $G_0$ as an upper bound and 1 as lower bound. Then in each iteration, it removes all vertices with query distance more than the average of upper and lower bounds. Then in the resulted graph $G_i$ we remove edges/vertices to maintain $G_i$ as a $(k, \lambda)$-FirmCore (lines 7 and 8). If $G_i$ is not empty, then we find a $(k, \lambda)$-FirmCore with query distance no more than maximum query distance of $dist_{G_i}$, so we change the upper bound. If $G_i$ is empty, then we need to change the lower bound. Finally, the algorithm terminates and returns a subgraph $G^*$, where $G^* \in \{ G_0, G_1, \dots, G_{i - 1} \}$ with the smallest query distance, $dist_{G_i}(V[G_i], Q)$. The time complexity of this algorithm is the same as FCCS-Global algorithm but the total number of iterations, $t$, is bounded by $\mathcal{O}(\log d_0)$, where $d_0 = dist_{G_0}(G_0, Q)$.

\head{FTCS Binary Search Algorithm}
The overall procedure of the FTCS Binary Search algorithm is exactly the same as Algorithm~\ref{alg:binary_search} when in lines 1 and 8 we use FirmTruss structure instead of FirmCore.






\subsubsection{Online Local Search Algorithms}
The Global algorithm finds the FirmCommunity (FirmCore and FirmTruss) in a top-down manner. In this section, we present another algorithm, called Local, which works in a bottom-up manner. 

%%%%%%%%%% Online Local Algorithm %%%%%%%%%% 
\input{Text/Algorithm_online_local_search}

\head{FCCS Local Algorithm}
Algorithm~\ref{alg:local_search} shows the details of the FCCS Local algorithm. It first computes the maximal $(k, \lambda)$-FirmCore using Algorithm~\ref{alg:FirmCore_G0} (line 1). It collects all vertices whose query distances are no greater than $i$ into $V'$ (line 4), and then constructs $G'$ as the induced subgraph of $G$ by $V'$ (line 5). Next, the algorithm examines whether $G'$ contains a $(k, \lambda)$-FirmCore whose query distance is $i$. If such a FirmCore exists, it is returned as the solution and otherwise, the algorithm increases $i$ by 1 for a new iteration.


\begin{theorem}[FCCS-Local Quality Approximation]\label{theorem:FCCS-local-approx-FCCS}
Algorithm~\ref{alg:local_search} achieves 2-approximation to an optimal solution $G[H^*]$ of the FCCS problem, that is, the obtained $(k, \lambda)$-FirmCore, $G[H]$, has \begin{equation*}
    diam(G[H])\leq 2 \times diam(G[H^*]).
\end{equation*}
\end{theorem}

\begin{proof}
By contradiction, we first show that $dist_{G[H]}(H, Q) \leq dist_{G[H^*]}(H^*, Q)$. Let $dist_{G[H]}(H, Q) > dist_{G[H^*]}(H^*, Q)$, so there exists another FirmCore with smallest diameter, so when $i = \\dist_{G[H^*]}(H^*, Q)$, the algorithm must find a FirmCore with query distance of $i$, which is contradiction as $i = dist_{G[H]}(H, Q)$ is the smallest value of $i$ that the algorithm finds a non-empty FirmCore. Thus, $dist_{G[H]}(H, Q) \leq dist_{G[H^*]}(H^*, Q)$. Based on triangle inequality, $diam(G[H]) \leq 2dist_{G[H]}(H, Q)$. Overall:
\begin{equation*}
    diam(G[H]) \leq 2dist_{G[H]}(H, Q) \leq 2 dist_{G[H^*]}(H^*, Q).
\end{equation*}
\end{proof}


\begin{theorem}[FCCS-Local Complexity]
Algorithm~\ref{alg:global_search} takes\\ $\mathcal{O}(\gamma(|V_0| + |E_0|)+|V|\lambda\log|L|+(|V|+|E|)|L|)$ time, and $\mathcal{O}(|V||L| + |E|)$ space, where $\gamma = dist_{G_0}(G_0, Q)$, $V_0$ and $E_0$ are the vertex set and edge set of $G_0$. 
\end{theorem}
\begin{proof}
The proof is similar to analysis of time complexity of Algorithm~\ref{alg:global_search}.
\end{proof}



\head{FTCS Local Algorithm}
The overall procedure of the FTCS Local algorithm is exactly the same as Algorithm~\ref{alg:local_search} when in lines 1, 6, and 16 we use FirmTruss structure instead of FirmCore.

\begin{theorem}[FTCS-Local Quality Approximation]
FTCS Local algorithm achieves 2-approximation to an optimal solution $G[H^*]$ of the FTCS problem, that is, the obtained $(k, \lambda)$-FirmCore, $G[H]$, has \begin{equation*}
    diam(G[H])\leq 2 \times diam(G[H^*]).
\end{equation*}
\end{theorem}
\begin{proof}
The proof is similar to the proof of Theorem~\ref{theorem:FCCS-local-approx-FCCS}
\end{proof}


\begin{theorem}[FTCS-Local Complexity]
FTCS-Global algorithm takes $\mathcal{O}(\gamma (|Q| |E_0| + \sum_{\ell \in L} |E_\ell|^{1.5}) + |E||L| + |E|\lambda \log |L|)$ time, and $\mathcal{O}(|E||L|)$ space, where $\gamma = dist_{G_0}(G_0, Q)$ and $E_0$ is the edge set of $G_0$.
\end{theorem}
\begin{proof}
The proof is similar to analysis of time complexity of FTCS-Global algorithm.
\end{proof}




\subsubsection{Index-based Algorithms}
Both Global and Local need to retrieve the maximal FirmCore (FirmTruss). However, computing the maximal FirmCore (FirmTruss) online from scratch is very inefficient for large multilayer networks. Actually, all the possible maximal FirmCore and FirmTruss of a given multilayer graph are determined, which can be precomputed and stored in an index for speeding up our algorithms. Motivated by this, in this section, we discuss how to employ FirmCore and FirmTruss decomposition to accelerate our algorithms.



\begin{dfn}[Index Dominance]
Given two indices $(k_1, \lambda_1)$ and $(k_2, \lambda_2)$, we say $(k_1, \lambda_1)$ dominates $(k_2, \lambda_2)$, denoted as $(k_2, \lambda_2) \prec (k_1, \lambda_1)$, if and only if \textbf{(1)} $k_1 \geq k_2$ and $\lambda_1 > \lambda_2$, or \textbf{(2)} $k_1 > k_2$ and $\lambda_1 \geq \lambda_2$.
\end{dfn}

\begin{dfn}[Skyline FirmCoreness]
Given a vertex $u \in V$, and $FC(u)$ including all the FirmCore indices $(k_i, \lambda_i)$ that $u$ is in $(k_i, \lambda_i)$-FirmCore. The skyline FirmCoreness of $u$, denoted as $\sfc{u}$ contains the FirmCore indices that are not dominated by others: 
\begin{equation*}
    \sfc{u} = \{ (k_i, \lambda_i) \in FC(u) | \nexists (k_j, \lambda_j):  (k_i, \lambda_i) \prec (k_j, \lambda_j) \}.
\end{equation*}
\end{dfn}

\begin{dfn}[Skyline FirmTrussness]
Given an edge schema $\varphi \in \mathcal{E}$, and $FT(u)$ including all the FirmTruss indices $(k_i, \lambda_i)$ that $\varphi$ is in $(k_i, \lambda_i)$-FirmTruss. The skyline FirmTrussness of $\varphi$, denoted as $\sft{\varphi}$ contains the FirmTruss indices that are not dominated by others: 
\begin{equation*}
    \sft{\varphi} = \{ (k_i, \lambda_i) \in FT(\varphi) | \nexists (k_j, \lambda_j):  (k_i, \lambda_i) \prec (k_j, \lambda_j) \}.
\end{equation*}
\end{dfn}

Based on the FirmCore and FirmTruss decomposition algorithms, we can easily find all indices that a vertex or an edge schema belongs to. Accordingly, we can find all skyline indices (edge schema) for each node.  Algorithm~\ref{alg:maximal_firmcore_index} shows the procedure of finding maximal FirmCore by using skyline indexing. The algorithm starts from query nodes and for each neighbour check whether that node has a skyline index that dominates the input $k, \lambda$. Similarly, Algorithm~\ref{alg:maximal_firmtruss_index} shows the corresponding procedure for finding the maximal FirmTruss.

\input{Text/Algorithm_Maximal_FirmCore_Index}
\input{Text/Algorithm_Maximal_FirmTruss_Index}

\begin{theorem}
Algorithm~\ref{alg:maximal_firmcore_index} takes $\mathcal{O}(m)$ time. 
\end{theorem}

The time complexity of Algorithm~\ref{alg:maximal_firmtruss_index} is the same as the time complexity of Algorithm~\ref{alg:maximal_firmcore_index}. 

\subsubsection{Improved Hybrid Algorithm}


%%%%%%%%%% Online Hybrid Algorithm %%%%%%%%%% 
Here, we propose a hybrid approach that takes the advantages of indexing,  local search, and optimizing by binary search. We use the idea of the Local algorithm. First, we use 1 as our lower bound of query distance and the query distance of G as the upper bound. We then, in each iteration, consider the induced subgraph of all nodes with query distance lower than the average of lower bound and upper bound. Then we maintain the subgraph as FirmCore (FirmTruss). If we find a solution, we change our upper bound to this case and repeat the process. If we find no solution, then we change our lower bound. This approach can significantly decrease the number of iterations. The details of this procedure can be seen in Algorithm~\ref{alg:hybrid_search}.

\input{Text/Algorithm_improved_hybrid_search}












\subsection{Comparison of Community Search Models in Multilayer Networks}\label{sec:compare_community_models}
In this section, we compare FirmCore and FirmTruss with the existing models of community search in multilayer networks and highlight their advantages. Table~\ref{tab:comparision_Table} shows the summary of theoretical comparison of structures used in existing models in terms of four main metrics, i.e., cohesiveness, connectivity, redundancy, scalability. Stars rank each model in terms of a metric.

\head{Cohesiveness}
Commonly in the literature, communities are identified as a subgraph for which the nodes are cohesive and densely connected internally with low communication cost. Accordingly, density and cohesiveness are important metrics to measure the quality of found communities. The ML $\mathbf{k}$-core model proposes an objective function for a trade-off between high density and the number of layers exhibiting high density. In this model, the minimum degree is considered as the density measure. Although there is no containment relationship between ML $\mathbf{k}$-core and FirmCore, it is experimentally shown that FirmCore can find subgraphs with higher density and higher average density per layer than the ML $\mathbf{k}$-core. ML-LCD model defines a community based on the fraction of the average number of edges inside and outside the subgraph. Although this model can find subgraphs with high density, it does not control the minimum degree within the subgraph, and one node may have degree 1. Finally, FirmTruss is more cohesive than FirmCore as each $(k, \lambda)$-FirmTruss is contained by $(k, \lambda)$-FirmCore.

\head{Connectivity}
Essentially, communities are considered as a connected subgraph. While ML  $\mathbf{k}$-core, ML-LCD community search model does not guarantee connectivity, our model based on FirmCore and FirmTruss forces the subgraph to be connected. Moreover, in the FirmCore, removing an edge may result in disconnectivity of the subgraph, but $(k, \lambda)$-FirmTruss guarantees that after removing at most $\lambda\times (k-1)$ inter-layer edges, the $(k, \lambda)$-FirmTruss is still connected.

\head{Redundancy}
In multilayer networks, the rich node connection information leads to redundancies, meaning that edges between the same pair of nodes repeatedly appear in different layers. Nodes with repeated connections are more likely to belong to the same community~\cite{Redundancy-ML-Community}. Also, without redundancy, the connection tightness between objects in multilayer networks may not be represented effectively and accurately. None of the ML $\mathbf{k}$-core, ML-LCD, and FirmCore guarantees edges' redundancy, while in $(k, \lambda)$-FirmTruss, we know that each edge has to appear in at least $\lambda$ layers. 

\head{Scalability}
Nowadays, many real networks contain millions or billions of vertices. As a result, the scalability of a method is a required property to apply to real big networks. In this section, we compare the scalability based on the time-complexity of algorithms. Our experimental results (Section~\ref{sec:experiments}) validate our theoretical comparison as well. Based on the exponential number of outputs in the ML k-core model, there is no polynomial-time algorithm to find the community based on this model. The time complexity of ML-LCD in the worst case is $\mathcal{O}(|V|^2 |C|^2|L|)$, where $|C|$ is the size of the subgraph, while the time complexity of FirmCore based is linear in the number of edges and nodes. Finally, the FirmTruss-based community search model takes $\mathcal{O}(|E|^{1.5})$ in the worst case. Therefore, based on the time complexity, FirmCore is more scalable than other methods, FirmTruss and ML-LCD may take $O(|V|^3)$ in the worst case, and finally, ML $\mathbf{k}$-core is exponential-time. 

\input{Text/Comparision_Table}




% \head{Robustness}



% \subsection{Parameter Selection}

% \head{Densest Community}



% \head{Most Diverse Community}





==> ProblemVariants.tex <==
\section{Problem Variants}
\label{sec:problem-variants}




==> Problem_Formulation.tex <==
\section{Problem Formulation}
\label{sec:Problem_Formulation}


